Permissionless Refereed Tournaments

Scalability problems in programmable blockchains have created a strong demand for secure methods that move the bulk of computation outside the blockchain. One of the preferred solutions to this problem involves off-chain computers that compete interactively to prove to the limited blockchain that theirs is the correct result of a given intensive computation. Each off-chain computer spends effort linear on the cost of the computation, while the blockchain adjudicates disputes spending only logarithmic effort. However, this effort is multiplied by the number of competitors, rendering disputes that involve a significant number of parties impractical and susceptible to Sybil attacks. In this paper, we propose a practical dispute resolution algorithm by which a single honest competitor can win disputes while spending effort linear on the cost of the computation, but only logarithmic on the number of dishonest competitors. This algorithm is a novel, stronger primitive for building permissionless fraud-proof protocols, which doesn't rely on complex economic incentives to be enforced.

==> Makefile <==
.PHONY: lin win mac clean test

SHELL=bash

all: nxn.pdf

nxn.bbl: nxn.bib
	pdflatex -halt-on-error -draftmode nxn
	bibtex nxn
	pdflatex -halt-on-error -draftmode nxn

nxn.pdf: nxn.tex nxn.bbl
	pdflatex -halt-on-error nxn

letter.pdf: letter.tex
	pdflatex -halt-on-error letter

bib:
	touch nxn.bib

clean:
	\rm *.aux *.bbl *.blg *.brf *.lbl *.log *~ *.dvi *.pdf *.ps *.o

win: nxn.pdf
	cmd /c start nxn.pdf

mac: nxn.pdf letter.pdf
	open nxn.pdf letter.pdf

lin: nxn.pdf
	xdg-open nxn.pdf &> /dev/null


